TweetCOVID: A System for Analyzing Public Sentiments and Discussions about COVID-19 via Twitter Activities

The COVID-19 pandemic has created widespread health and economical impacts, affecting millions around the world. To better understand these impacts, we present the TweetCOVID system that offers the capability to understand the public reactions to the COVID-19 pandemic in terms of their sentiments, emotions, topics of interest and controversial discussions, over a range of time periods and locations, using public tweets. We also present three example use cases that illustrates the usefulness of our proposed TweetCOVID system.

==> covidDemo-long.tex <==
@inproceedings{nielsen2011new,
  title={A new ANEW: Evaluation of a word list for sentiment analysis in microblogs},
  author={Nielsen, Finn {\AA}rup},
  booktitle={Workshop on'Making Sense of Microposts: Big things come in small packages},
  pages={93--98},
  year={2011}
}

@inproceedings{mohammad2013nrc,
  title={NRC-Canada: Building the State-of-the-Art in Sentiment Analysis of Tweets},
  author={Mohammad, Saif and Kiritchenko, Svetlana and Zhu, Xiaodan},
  booktitle={Second Joint Conference on Lexical and Computational Semantics (* SEM), Volume 2: Proceedings of the Seventh International Workshop on Semantic Evaluation (SemEval 2013)},
  pages={321--327},
  year={2013}
}

@incollection{plutchik1980general,
  title={A general psychoevolutionary theory of emotion},
  author={Plutchik, Robert},
  booktitle={Theories of emotion},
  pages={3--33},
  year={1980},
  publisher={Elsevier}
}

@article{blei2003latent,
  title={Latent dirichlet allocation},
  author={Blei, David M and Ng, Andrew Y and Jordan, Michael I},
  journal={Journal of machine Learning research},
  volume={3},
  number={Jan},
  pages={993--1022},
  year={2003}
}

@article{su2020examining,
  title={Examining the impact of COVID-19 lockdown in Wuhan and Lombardy: A psycholinguistic analysis on Weibo and twitter},
  author={Su, Yue and Xue, Jia and Liu, Xiaoqian and Wu, Peijing and Chen, Junxiang and Chen, Chen and Liu, Tianli and Gong, Weigang and Zhu, Tingshao},
  journal={International Journal of Environmental Research and Public Health},
  volume={17},
  number={12},
  pages={4552},
  year={2020},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{vicari2020covid19,
  title={One Platform, a Thousand Worlds: On Twitter Irony in the Early Response to the COVID-19 Pandemic in Italy},
  author={Vicari, Stefania and Murru, Maria Francesca},
  journal={Social Media+ Society},
  volume={6},
  number={3},
  pages={2056305120948254},
  year={2020},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{gruzd2020going,
  title={Going viral: How a single tweet spawned a COVID-19 conspiracy theory on Twitter},
  author={Gruzd, Anatoliy and Mai, Philip},
  journal={Big Data \& Society},
  volume={7},
  number={2},
  pages={2053951720938405},
  year={2020},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{stephens2020geospatial,
  title={A geospatial infodemic: Mapping Twitter conspiracy theories of COVID-19},
  author={Stephens, Monica},
  journal={Dialogues in Human Geography},
  volume={10},
  number={2},
  pages={276--281},
  year={2020},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{fornacciari2018holistic,
  title={A holistic system for troll detection on Twitter},
  author={Fornacciari, Paolo and Mordonini, Monica and Poggi, Agostino and Sani, Laura and Tomaiuolo, Michele},
  journal={Computers in Human Behavior},
  volume={89},
  pages={258--268},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{chatzakou2017mean,
  title={Mean birds: Detecting aggression and bullying on twitter},
  author={Chatzakou, Despoina and Kourtellis, Nicolas and Blackburn, Jeremy and De Cristofaro, Emiliano and Stringhini, Gianluca and Vakali, Athena},
  booktitle={Proceedings of the 2017 ACM on web science conference},
  pages={13--22},
  year={2017}
}

@inproceedings{lim2018rapid,
  title={RAPID: Real-time Analytics Platform for Interactive Data Mining},
  author={Lim, Kwan Hui and Jayasekara, Sachini and Karunasekera, Shanika and Harwood, Aaron and Falzon, Lucia and Dunn, John and Burgess, Glenn},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={649--653},
  year={2018},
  organization={Springer}
}

@article{comito2019bursty,
  title={Bursty event detection in Twitter streams},
  author={Comito, Carmela and Forestiero, Agostino and Pizzuti, Clara},
  journal={ACM Transactions on Knowledge Discovery from Data (TKDD)},
  volume={13},
  number={4},
  pages={1--28},
  year={2019},
  publisher={ACM New York, NY, USA}
}


@inproceedings{kwan2020covid,
	AUTHOR = {Jolin Shaynn-Ly Kwan and Kwan Hui Lim},
	TITLE = {{Understanding Public Sentiments, Opinions and Topics about COVID-19 using Twitter}},
	BOOKTITLE = {{Proceedings of the 2020 IEEE/ACM International Conference on Advances in Social Networks Analysis and Mining (ASONAM'20)}},
	YEAR = {2020}
}

@inproceedings{wang2018happiness,
  title={Happiness is a choice: sentiment and activity-aware location recommendation},
  author={Wang, Jia and Feng, Yungang and Naghizade, Elham and Rashidi, Lida and Lim, Kwan Hui and Lee, Kate},
  booktitle={Companion Proceedings of the The Web Conference 2018},
  pages={1401--1405},
  year={2018}
}

@inproceedings{madisetty2019event,
  title={Event Recommendation using Social Media},
  author={Madisetty, Sreekanth},
  booktitle={2019 IEEE 35th International Conference on Data Engineering (ICDE)},
  pages={2106--2110},
  year={2019},
  organization={IEEE}
}

@inproceedings{jonsson2015evaluation,
  title={An evaluation of topic modelling techniques for twitter},
  author={J{\'o}nsson, El{\i}as and Stolee, Jake},
  year={2015}
}

@article{abdelhaq2013eventweet,
  title={Eventweet: Online localized event detection from twitter},
  author={Abdelhaq, Hamed and Sengstock, Christian and Gertz, Michael},
  journal={Proceedings of the VLDB Endowment},
  volume={6},
  number={12},
  pages={1326--1329},
  year={2013},
  publisher={VLDB Endowment}
}
